IFCap: Image-like Retrieval and Frequency-based Entity Filtering for Zero-shot Captioning

Recent advancements in image captioning have explored text-only training methods to overcome the limitations of paired image-text data. However, existing text-only training methods often overlook the modality gap between using text data during training and employing images during inference. To address this issue, we propose a novel approach called Image-like Retrieval, which aligns text features with visually relevant features to mitigate the modality gap. Our method further enhances the accuracy of generated captions by designing a Fusion Module that integrates retrieved captions with input features. Additionally, we introduce a Frequency-based Entity Filtering technique that significantly improves caption quality. We integrate these methods into a unified framework, which we refer to as IFCap ($\textbf{I}$mage-like Retrieval and $\textbf{F}$requency-based Entity Filtering for Zero-shot $\textbf{Cap}$tioning). Through extensive experimentation, our straightforward yet powerful approach has demonstrated its efficacy, outperforming the state-of-the-art methods by a significant margin in both image captioning and video captioning compared to zero-shot captioning based on text-only training.

==> tables/ablation13_retrieval_datastore_combination.tex <==
\begin{table}[t]
\tabcolsep=3pt
\resizebox{\columnwidth}{!}{
\begin{tabular}{l|c|cc|cc|cc|cc}
\toprule[2pt]
\multirow{3}{*}{\textbf{Datastore}} & \multirow{3}{*}{\textbf{EF}} & \multicolumn{8}{c}{\textbf{COCO $\Longrightarrow$ NoCaps Val}} \\
                                    & & \multicolumn{2}{c|}{In} & \multicolumn{2}{c|}{Near} & \multicolumn{2}{c|}{Out} & \multicolumn{2}{c}{Entire} \\
                                    & & \multicolumn{1}{c}{C} & \multicolumn{1}{c|}{S} & \multicolumn{1}{c}{C} & \multicolumn{1}{c|}{S} & \multicolumn{1}{c}{C} & \multicolumn{1}{c|}{S} & \multicolumn{1}{c}{C} & \multicolumn{1}{c}{S} \\ 
\midrule
\multirow{2}{*}{CC3M}          & $\checkmark$ & & & & & & & &  \\
                               &              & & & & & & & &  \\
\midrule
\multirow{2}{*}{CC3M + COCO}   & $\checkmark$ & & & & & & & &  \\
                               &              & & & & & & & &  \\
\midrule
\multirow{2}{*}{COCO}          & $\checkmark$ & 75.8 & 12.4 & 72.3 & 11.6 & 60.2 & 8.9 & 70.5 & 10.8  \\
                               &              & 70.1 & 11.2 & 72.5 & 10.9 & 72.1 & 9.6 & 74.0 & 10.5  \\
\bottomrule[2pt]
\end{tabular}
}\caption{ablation 13}\label{tb:ablation13}
\end{table}





==> tables/ablation3_text_corpus_quantity.tex <==
\begin{table}[t]
\tabcolsep=3pt
\resizebox{\columnwidth}{!}{
\begin{tabular}{c|c|cccc|cccc}
\toprule[2pt]
\multirow{2}{*}{Data} & \multirow{2}{*}{Method} & \multicolumn{4}{c}{\textbf{COCO}} & \multicolumn{4}{|c}{\textbf{NoCaps val}} \\
                     &                        & B@4 & M & C & S & In & Near & Out & All \\
\midrule
\multirow{2}{*}{\text{0.1\%}} & ViECap  & - & - & 32.2 & - & 20.9 & 27.6 & 34.9 & 30.2 \\
                                 & \model & & & & & & & & \\
\midrule
\multirow{2}{*}{\text{1\%}}   & ViECap & - & - & 63.9 & - & 34.6 & 39.9 & 39.3 & 40.4 \\
                                 & \model & & & & & & & & \\
\midrule
\multirow{2}{*}{\text{10\%}}  & ViECap & - & - & 83.6 & - & 45.9 & 51.8 & 48.7 & 53.3 \\
                                 & \model & & & & & & & & \\
\midrule
\multirow{2}{*}{\text{100\%}} & ViECap & 27.2 & 24.8 & 92.9 & 18.2 & 61.1 & 64.3 & 65.0 & 66.2 \\
                              & \model & 30.3 & 26.5 & 107.2 & 20.3 & 70.1 & 72.5 & 72.1 & 74.0 \\
\bottomrule[2pt]
\end{tabular}
}\caption{ablation 3}\label{tb:ablation_corpus_quantity}
\end{table}

==> tables/ablation4_text_corpus_domain.tex <==
\begin{table}[t]
\tabcolsep=3pt
\resizebox{\columnwidth}{!}{
\begin{tabular}{c|cccc|cccc}
\toprule[2pt]
\multirow{2}{*}{Dataset} & \multicolumn{4}{c}{\textbf{COCO}} & \multicolumn{4}{|c}{\textbf{Flickr30k}} \\
                      & B@4 & M & C & S & B@4 & M & C & S  \\
\midrule
CC3M  & & & & & & & & \\
SS1M  & & & & & & & & \\
COCO  & 30.8 & 26.7 & 108.0 & 20.3 & 23.5 & 23.0& 64.4 & 17.0 \\
\bottomrule[2pt]
\end{tabular}
}\caption{ablation 4}\label{tb:ablation_corpus_different_domain}
\end{table}

==> tables/ablation5_add_image_pair.tex <==
\begin{table}[t]
\tabcolsep=3pt
\resizebox{\columnwidth}{!}{
\begin{tabular}{c|cccc|cccc}
\toprule[2pt]
\multirow{2}{*}{Model}  &  \multicolumn{4}{c}{\textbf{COCO}} & \multicolumn{4}{|c}{\textbf{NoCaps val}} \\
                       &  B@4 & M & C & S & In & Near & Out & All \\
\midrule
\multicolumn{9}{l}{Supervised learning} \\
ClipCap & & & & & & & & \\
\midrule
\multirow{2}{*}{Data}  &  \multicolumn{4}{c}{\textbf{COCO}} & \multicolumn{4}{|c}{\textbf{NoCaps val}} \\
                       &  B@4 & M & C & S & In & Near & Out & All \\
\midrule

\text{0.1\%}  & & & & & & & & \\
\text{1\%}  & & & & & & & & \\
\text{10\%}  & & & & & & & & \\
\text{100\%}  & & & & & & & & \\
\bottomrule[2pt]
\end{tabular}
}\caption{ablation 5}\label{tb:ablation_image_pair}
\end{table}

==> tables/ablation7_language_model_freeze.tex <==
\begin{table}[t]
\tabcolsep=3pt
\resizebox{\columnwidth}{!}{
\begin{tabular}{c|cccc|cccc}
\toprule[2pt]
Freeze  & \multicolumn{4}{c|}{\textbf{COCO}} & \multicolumn{4}{c}{\textbf{NoCaps val}} \\
Decoder & B@4 & M & C & S & In & Near & Out & All \\
\midrule
$\checkmark$ & & & & & & & & \\
             & & & & & & & & \\
\bottomrule[2pt]
\end{tabular}
}\caption{ablation 7}\label{tb:ablation_freeze_decoder}
\end{table}

